Thompson Sampling with Diffusion Generative Prior

In this work, we initiate the idea of using denoising diffusion models to learn priors for online decision making problems. Our special focus is on the meta-learning for bandit framework, with the goal of learning a strategy that performs well across bandit tasks of a same class. To this end, we train a diffusion model that learns the underlying task distribution and combine Thompson sampling with the learned prior to deal with new tasks at test time. Our posterior sampling algorithm is designed to carefully balance between the learned prior and the noisy observations that come from the learner's interaction with the environment. To capture realistic bandit scenarios, we also propose a novel diffusion model training procedure that trains even from incomplete and/or noisy data, which could be of independent interest. Finally, our extensive experimental evaluations clearly demonstrate the potential of the proposed approach.

==> algorithms/meta-bandits.tex <==
\begin{algorithm}[htb]
    \caption{Meta-learning for Bandits with Diffusion Models}
    \label{algo:MetaBandits}
\begin{algorithmic}[1]
    \STATE \uline{\texttt{Meta-Training Phase: a) Train Diffusion Model}}
    \vspace{0.1em}
    \STATE {\bfseries Input:}
     Training set (either clean $\trainset$ or imperfect $\trainsetdeg$) of expected rewards $(\vtask[\meanreward])_{\task}$ from different tasks $\task\sim\taskdistribution$
     
     
    \STATE Train a diffusion model $\denoiser_{\param}$ to model the distribution of the mean rewards (use \cref{algo:training-imperfect} in the case of imperfect dataset $\trainsetdeg$)
    \vspace{0.1em}
    \STATE \uline{\texttt{Meta-Training Phase: b) Variance Calibration}}
    \vspace{0.1em}
    \STATE {\bfseries Input:}
     Calibration set (either clean $\calset$ or imperfect $\calsetdeg$) of expected rewards $(\vtask[\meanreward])_{\task}$ from different tasks $\task\sim\taskdistribution$
    \STATE Estimate the mean squared reconstruction error $(\vdiff[\diffbackdev])_{\diffstep\in\intinterval{1}{\nDiffsteps}}$ for the model $\denoiser_{\param}$ at different noise levels with either \cref{algo:var-calib} to calibrate the variance  (use \cref{algo:var-calib-imperfect}  in the case of imperfect dataset $\calsetdeg$)
    \vspace{0.1em}
    \STATE \uline{\texttt{{Meta-Deployment Phase}}
    \vspace{0.1em}
    \STATE \todos{{\bfseries Input:}}
    \STATE For any new task $\task$, run Thompson sampling with diffusion prior (\cref{algo:DiffTS}) with trained model
\end{algorithmic}
\end{algorithm}


==> algorithms/post-sampling-deprecated.tex <==
\begin{algorithm}[htb]
    \caption{Posterior Sampling with Diffusion Prior}
    \label{algo:post-sampling}
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} Observation $\vdiff[\obs][0]\in\R^{\nArms}$, 
    noise standard deviation $\noisedev\in\R^{\nArms}$,
    binary mask $\mask\in\{0,1\}^{\nArms}$,
    diffusion model $\denoiser_{\param}$ and associated reconstruction errors $(\vdiff[\diffbackdev])_{\diffstep\in\intinterval{1}{\nDiffsteps}}$
    \STATE {\bfseries Output:}
    Posterior sample $\vdiff[\latent][0]$ (resp. $\vdiff[\latent][\intintervalalt{0}{\nDiffsteps}]$) approximately sampled from $\vdiff[\rvlat][0]\given\vdiff[\obs][0]$
    (resp. $\vdiff[\rvlat][\intintervalalt{0}{\nDiffsteps}]\given\vdiff[\obs][0]$)
    \vspace{0.2em}
    \STATE Sample $\vdiff[\latent][\nDiffsteps]\sim\gaussian(0,\Id)$
    \FOR{$\diffstep \in \nDiffsteps-1, \ldots, 0$}
    \STATE Predict clean sample $\vdiff[\est{\latent}][0]=\denoiser_{\param}(\vdupdate[\latent],\diffstep+1)$ and associated noise $\vdupdate[\bar{\noise}]$
    % \Statex \hspace{1.5em} \(\triangleright\) optionally, sample $\vdupdate[\bar{\noise}]$ from $\gaussian(0,\Id)$
    \STATE Compute diffused observation
    $\vdiff[\tilde{\obs}]    =\sqrt{\vdiff[\diffscalingprod]}\vdiff[\obs][0]
    + \sqrt{1-\vdiff[\diffscalingprod]}\vdupdate[\bar{\noise}]$
    \FOR{$\arm\in\arms$}
    \STATE If $\mask=0$, sample $\vadiff[\latent][\arm]\sim\density_{\param,\diffbackdev}(\vadiff[\rvlat]\given\vdupdate[\latent])$
    \STATE If $\mask=1$, sample
    \[\vadiff[\latent][\arm]\sim
    \tilde{\densityalt}(
        \vadiff[\rvlat]\given\vdupdate[\latent],\vdiff[\obs][0]
        )
        \,\propto\,
        \density_{\param,\diffbackdev}(\vadiff[\rvlat]\given\vdupdate[\latent])
        \,
        \gaussian
        \big(
        \vadiff[\rvlat]
        \,;\,\vadiff[\tilde{\obs}],
        \vdiff[\diffscalingprod]
        ((\va[\noisedev])^2 +
        \vdiff[\backvarscaling](\vadupdate[\diffbackdev])^2
    \big)\]
    \ENDFOR
    \ENDFOR
\end{algorithmic}
\end{algorithm}


==> appendices/apx-pseudocodes.tex <==
\input{algorithms/meta-bandits}
\input{algorithms/var-calib}
\input{algorithms/diffts}
\input{algorithms/var-calib-imperfect}
\input{algorithms/training-imperfect}
